Learning to Prove from Synthetic Theorems

A major challenge in applying machine learning to automated theorem proving is the scarcity of training data, which is a key ingredient in training successful deep learning models. To tackle this problem, we propose an approach that relies on training with synthetic theorems, generated from a set of axioms. We show that such theorems can be used to train an automated prover and that the learned prover transfers successfully to human-generated theorems. We demonstrate that a prover trained exclusively on synthetic theorems can solve a substantial fraction of problems in TPTP, a benchmark dataset that is used to compare state-of-the-art heuristic provers. Our approach outperforms a model trained on human-generated problems in most axiom sets, thereby showing the promise of using synthetic data for this task.

==> more_background.tex <==
\section{First-Order Logic}
\needcite{FOL book}

First-order logic is a formal language to write \emph{formulas} and prove whether they are true or false using \emph{inference rules} and \emph{axioms} (axiomatic formulas assumed true to start with).

A formula is composed of 
a) constants such as \texttt{alice} or the number 3,
b) functions such as \texttt{plus(3, 4)} or \texttt{successor(four)} whose ranges 
are arbitrary,
c) predicates which are functions with range \{\texttt{true}, \texttt{false}\},
d) variables such as $X$ and $Y$ which are placeholders which value is not specified
and can be \emph{substituted} with some formula,
e) quantifiers over variables (for all $\forall$, there exists $\exists$),
and finally f) logical connectives such as 'or' $\lor$, 'and' $\land$', 'not' $\lnot$, 'implies' $\rightarrow$, 'equivalent' $\leftrightarrow$.
For example,
\texttt{$\forall$ X, human(X) $\rightarrow \exists$ Y, parent(Y, X)} is a formula.
\comment{L: `|' or `$\lor$'?}

By convention we write function, predicate and constant symbols in lower cases,
and variables with a starting uppercase letter.

An inference rule (such as \emph{resolution} described below) takes one or more formulas and produces a new formula which is true if the first two formulas are true.


\subsection{Resolution calculus}

The basic unit of the resolution calculus is the \emph{clause}, 
which is a formula that contain only universally quantified variables (no existential quantifier),
and is composed of a \emph{disjunction} (using only $\lor$ and $\lnot$) of \emph{literals}, which are predicates, which arguments can be constants, variables, or functions.
The universal quantifiers are omitted.
For example
\texttt{$\lnot$parent(X, bob) $\lor$ $\lnot$ parent(bob, charlotte) $\lor$ grand\_parent(X, charlotte)}
is a clause that can be written as a formula (using De Morgan's law)
\texttt{$\forall$ X, parent(X, bob) $\land$ parent(bob, charlotte) $\rightarrow$ grand\_parent(X, charlotte)}.

A formulas is said to be in Conjunctive Normal Form (CNF) if it is made of a conjunction ($\land$) of clauses.

\comment{V: I don't think it is necessary to mention axioms in this section.}


